Task-Specific Adaptation with Restricted Model Access

The emergence of foundational models has greatly improved performance across various downstream tasks, with fine-tuning often yielding even better results. However, existing fine-tuning approaches typically require access to model weights and layers, leading to challenges such as managing multiple model copies or inference pipelines, inefficiencies in edge device optimization, and concerns over proprietary rights, privacy, and exposure to unsafe model variants. In this paper, we address these challenges by exploring "Gray-box" fine-tuning approaches, where the model's architecture and weights remain hidden, allowing only gradient propagation. We introduce a novel yet simple and effective framework that adapts to new tasks using two lightweight learnable modules at the model's input and output. Additionally, we present a less restrictive variant that offers more entry points into the model, balancing performance with model exposure. We evaluate our approaches across several backbones on benchmarks such as text-image alignment, text-video alignment, and sketch-image alignment. Results show that our Gray-box approaches are competitive with full-access fine-tuning methods, despite having limited access to the model.

==> tables/ablations.tex <==
% \begin{table}[ht]
% \centering
% \small
% % \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}l|llll@{}}
% \toprule
% Model & R@1 & R@5 & R@10 & R@50 \\ \midrule
% Original (zero-shot) & 47.04 & 74.18 & 83.10 & 96.36 \\ \midrule
% {[}Input{]} Txt & 49.56 & 75.74 & 84.88 & 96.96 \\
% {[}Input{]} Vis & 49.04 & 75.54 & 84.18 & 96.86 \\
% {[}Input{]} Txt \& Vis & 50.56 & 76.84 & 85.40 & 97.04 \\
% {[}Output{]} Txt & 51.26 & 77.90 & 85.60 & 97.38 \\
% {[}Output{]} Vis & 51.48 & 78.04 & 86.00 & 97.52 \\
% {[}Output{]} Txt \& Vis & 51.54 & 78.46 & 86.16 & 97.46 \\ \midrule
% Ours & \textbf{52.12} & \textbf{78.96} & \textbf{86.84} & \textbf{97.54} \\ \bottomrule
% \end{tabular}
%   % }

% \caption{Ablation study on the COCO 5k validation set, with the CLIP model encoders.
% \rami{What about the ablation on the noise?}}
% % \vspace{-1em}
% \label{tab:ablation}
% \end{table}

\begin{table}[ht]
\centering
\small
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccllll}
\hline
 & \multicolumn{4}{c}{Adapters} & \multicolumn{4}{c}{Results} \\
 & \multicolumn{2}{c}{Input} & \multicolumn{2}{c}{Output} & \multicolumn{4}{c}{Recall@K} \\
\multicolumn{1}{c}{Baseline} & Vision & \multicolumn{1}{c|}{Text} & Vision & \multicolumn{1}{c|}{Text} & R@1 & R@5 & R@10 & R@50 \\ \hline
Original (ZS) & \xmark & \multicolumn{1}{c|}{\xmark} & \xmark & \multicolumn{1}{c|}{\xmark} & 47.04 & 74.18 & 83.10 & 96.36 \\
Full FT & - & \multicolumn{1}{c|}{-} & - & \multicolumn{1}{c|}{-} & 53.06 & 79.32 & 87.58 & 97.62 \\
LoRA & - & \multicolumn{1}{c|}{-} & - & \multicolumn{1}{c|}{-} & 53.48 & 79.78 & 87.46 & 97.60 \\ \hline
\ours-Itxt & \xmark & \multicolumn{1}{c|}{\cmark} & \xmark & \multicolumn{1}{c|}{\xmark} & 49.90 & 76.02 & 84.96 & 97.08 \\
\ours-Ivis & \cmark & \multicolumn{1}{c|}{\xmark} & \xmark & \multicolumn{1}{c|}{\xmark} & 49.40 & 75.54 & 84.42 & 97.00 \\
\ours-I & \cmark & \multicolumn{1}{c|}{\cmark} & \xmark & \multicolumn{1}{c|}{\xmark} & 50.70 & 76.74 & 85.16 & 97.02 \\
\ours-Otxt & \xmark & \multicolumn{1}{c|}{\xmark} & \xmark & \multicolumn{1}{c|}{\cmark} & 51.22 & 77.94 & 86.02 & 97.32 \\
\ours-Ovis & \xmark & \multicolumn{1}{c|}{\xmark} & \cmark & \multicolumn{1}{c|}{\xmark} & 51.66 & 78.34 & 86.28 & 97.48 \\
\ours-O & \xmark & \multicolumn{1}{c|}{\xmark} & \cmark & \multicolumn{1}{c|}{\cmark} & 51.40 & 78.28 & 86.26 & 97.52 \\ \hline
\ours & \cmark & \multicolumn{1}{c|}{\cmark} & \cmark & \multicolumn{1}{c|}{\cmark} & \textbf{53.10} & \textbf{78.90} & \textbf{86.76} & \textbf{97.52} \\ \hline
\end{tabular}
  % }

\caption{Ablation study on the COCO 5k validation set, with the BLIP model encoders.
% \vspace{-1em}
\label{tab:ablation}
\end{table}



==> tables/blip_coco_flickr.tex <==
\begin{table}[ht]
\centering
\small

\caption{Results on two Text-to-Image Retrieval benchmarks, using the BLIP backbone.
}
\label{tab:blip_coco}
% \resizebox{0.9\columnwidth}{!}{%
\begin{tabular}{@{}lllllllll@{}}
\toprule
 & \multicolumn{4}{c}{COCO 5k} & \multicolumn{4}{c}{Flickr30K} \\
\multicolumn{1}{l|}{Model} & R@1 & R@5 & R@10 & \multicolumn{1}{l|}{R@50} & R@1 & R@5 & R@10 & R@50 \\ \midrule
\multicolumn{1}{l|}{Full FT} & 53.06 & 79.32 & {\ul 87.58} & \multicolumn{1}{l|}{97.62} & {\bf 87.3} & 96.5 & {\ul 98.1} & 99.4 \\
 \multicolumn{1}{l|}{Last Layers FT} & {\bf 54.32} & {\bf 80.32} & {\bf 87.66} & \multicolumn{1}{l|}{{\bf 97.68}} & {\ul 86.5} & {\bf 96.7} & {\bf 98.3} & {\bf 99.7} \\
 \multicolumn{1}{l|}{LoRA} & 53.48 & {\ul 79.78} & 87.46 & \multicolumn{1}{l|}{97.6} & 85.4 & {\ul 96.6} & {\ul 98.1} & {\ul 99.6} \\
\rowcolor{\rowlightgray} \multicolumn{1}{l|}{\ourspT} & {\ul 54.14} & 79.72 & 87.48 & \multicolumn{1}{l|}{{\ul 97.66}} & 84.7 & 95.9 & 97.7 & 99.4 \\
\rowcolor{\rowdarkgray} \multicolumn{1}{l|}{\oursT} & 53.18 & 79.14 & 87.04 & \multicolumn{1}{l|}{97.58} & 83.7 & 95.9 & 97.7 & 99.4 \\
\rowcolor{\rowblack} \multicolumn{1}{l|}{Linear Probing} & 51.4 & 78.28 & 86.26 & \multicolumn{1}{l|}{97.52} & 83.5 & 95.6 & 97.6 & 99.3 \\
\rowcolor{\rowblack} \multicolumn{1}{l|}{Original (zero-shot)} & 47.04 & 74.18 & 83.1 & \multicolumn{1}{l|}{96.36} & 78.5 & 94.5 & 96.8 & 98.9 \\
\bottomrule
\end{tabular}
  % }
\end{table}


==> tables/blip_videos.tex <==
\begin{table*}[ht]
\centering
\small
\label{tab:blip_video}
\resizebox{0.99\columnwidth}{!}{%
\begin{tabular}{lllllllll}
\hline
 & \multicolumn{4}{c}{MSR-VTT} & \multicolumn{4}{c}{VATEX} \\
\multicolumn{1}{l|}{Model} & R@1 & R@5 & R@10 & \multicolumn{1}{l|}{R@50} & R@1 & R@5 & R@10 & R@50 \\ \hline
\multicolumn{1}{l|}{Full Fine-tuning} & 35.96 & 63.96 & 74.28 & \multicolumn{1}{l|}{91.33} & {\bf 46.97} & {\bf 81.13} & {\bf 89.17} & {\bf 97.97} \\
 \multicolumn{1}{l|}{Last Layers FT} & 36.92 & 64.07 & {\ul 74.92} & \multicolumn{1}{l|}{{\ul 91.47}} & {\ul 44.47} & {\ul 78.33} & {\ul 87.3} & {\ul 97.37} \\
 \multicolumn{1}{l|}{LoRA} & {\bf 37.72} & {\bf 65.77} & {\bf 76.27} & \multicolumn{1}{l|}{{\bf 92.31}} & 41.63 & 75.43 & 84.43 & 96.5 \\
\rowcolor{\rowlightgray} \multicolumn{1}{l|}{\ourspT} & 37.04 & {\ul 64.14} & 74.29 & \multicolumn{1}{l|}{91.36} & 41.23 & 75.43 & 83.6 & 95.67 \\
\rowcolor{\rowdarkgray} \multicolumn{1}{l|}{\oursT} & {\ul 37.24} & 63.98 & 74.21 & \multicolumn{1}{l|}{91.34} & 41.03 & 73.2 & 82.8 & 95.53 \\
\rowcolor{\rowblack} \multicolumn{1}{l|}{Linear Probing} & 35.9 & 62.71 & 72.83 & \multicolumn{1}{l|}{90.63} & 38.33 & 70.53 & 80.97 & 94.4 \\
\rowcolor{\rowblack} \multicolumn{1}{l|}{Original (zero-shot)} & 32.14 & 56.53 & 66.38 & \multicolumn{1}{l|}{85.24} & 31.33 & 61.13 & 71.17 & 89.4 \\
\hline
\end{tabular}
  }
\end{table*}


==> tables/stanford_cars.tex <==
\begin{table}[ht]
\centering
% \small
\caption{Precision@K comparison on the Stanford-Cars dataset using the BLIP backbone. \ours is competitive with the strongest white-box baseline, Full Fine-Tuning, but both are outperformed by \oursp across most metrics.}

\label{tab:stanford_cars}
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}llllll@{}}
\toprule
 & P@1   & P@5   & P@10  & P@50  & P@70  \\ \midrule
Full Fine-tune & {\ul 98.07} & {\ul 98.08} & 97.76 & {\ul 77.64} & {\ul 57.55} \\
Last Layers Fine-tune & 95.03 & 95.8 & 95.99 & 76.02 & 57.13 \\
LoRa & 90.08 & 88.22 & 86.11 & 66.25 & 52.56 \\
\rowcolor{\rowlightgray} \ourspT & {\bf 98.45} & {\bf 98.21} & {\ul 97.87} & {\bf 77.78} & 57.54 \\
\rowcolor{\rowdarkgray} \oursT & 97.16 & 97.91 & {\bf 97.97} & 77.53 & {\bf 57.59} \\
\rowcolor{\rowblack} Linear Probing & 78.1 & 74.9 & 74.38 & 55.73 & 45.96 \\
\rowcolor{\rowblack}  Original (zero-shot) & 63.96 & 62.67 & 58.51 & 40.73 & 34.78 \\
\bottomrule
\end{tabular}
  % }
\end{table}


==> tables/sub_coco.tex <==
\begin{table*}[ht]
\centering
% \small
\caption{Performance comparison using the BLIP backbone on different COCO sub-domain splits. Each domain corpus was collected based on human-annotated objects within the images (number of training images in parentheses). Our adapters achieve performance on par with LoRA. The highest values are marked in {\bf bold}, and the second best are {\ul underlined}.}
\label{tab:sub_coco_blip}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lllllllllllll@{}}
\toprule
%
         & \multicolumn{3}{c}{Building {\scriptsize (23,021)}} & \multicolumn{3}{c}{Furniture {\scriptsize (17,882)}} & \multicolumn{3}{c}{Grass {\scriptsize (22,575)}} & \multicolumn{3}{c}{Metal {\scriptsize (22,526)}} \\
        \multicolumn{1}{l|}{} & R@1 & R@5 & \multicolumn{1}{l|}{R@10} & R@1 & R@5 & \multicolumn{1}{l|}{R@10} & R@1 & R@5 & \multicolumn{1}{l|}{R@10} & R@1 & R@5 & R@10 \\ \midrule
        
         \multicolumn{1}{l|}{Full Fine-tune} & 58.47 & 84.54 & \multicolumn{1}{l|}{91.18} & {\ul 62.51} & {\bf 88.59} & \multicolumn{1}{l|}{93.48} & 65.2 & 88.76 & \multicolumn{1}{l|}{94.97} & 61.8 & 85.2 & 91.53 \\
        
         \multicolumn{1}{l|}{Last Layers Fine-tune} & {\ul 60.06} & {\bf 85.73} & \multicolumn{1}{l|}{{\ul 91.77}} & {\bf 63.09} & 87.54 & \multicolumn{1}{l|}{{\ul 93.58}} & {\bf 68.42} & {\bf 91.43} & \multicolumn{1}{l|}{{\bf 95.82}} & 62.08 & {\bf 86.72} & 91.6 \\
        
         \multicolumn{1}{l|}{LoRA} & 59.66 & {\ul 84.74} & \multicolumn{1}{l|}{{\bf 92.07}} & 61.84 & {\ul 88.3} & \multicolumn{1}{l|}{93.48} & {\ul 67.02} & 89.94 & \multicolumn{1}{l|}{{\ul 95.61}} & {\bf 63.18} & {\ul 86.51} & {\bf 91.95} \\
        
        \rowcolor{\rowlightgray} \multicolumn{1}{l|}{\ourspT} & {\bf 60.26} & 84.14 & \multicolumn{1}{l|}{91.48} & 61.94 & 88.11 & \multicolumn{1}{l|}{{\bf 93.67}} & 65.42 & {\ul 90.58} & \multicolumn{1}{l|}{{\ul 95.61}} & {\ul 62.15} & 85.75 & {\ul 91.67} \\
        
        \rowcolor{\rowdarkgray} \multicolumn{1}{l|}{\oursT} & 58.57 & 83.94 & \multicolumn{1}{l|}{91.28} & 61.55 & 87.15 & \multicolumn{1}{l|}{91.85} & 65.42 & 90.26 & \multicolumn{1}{l|}{95.5} & 61.05 & 85.34 & 91.47 \\
        
        \rowcolor{\rowblack} \multicolumn{1}{l|}{Linear Probing} & 56.89 & 83.35 & \multicolumn{1}{l|}{90.98} & 60.98 & 86.1 & \multicolumn{1}{l|}{92.14} & 64.67 & 89.72 & \multicolumn{1}{l|}{94.97} & 59.26 & 84.65 & 90.64 \\
        
        \rowcolor{\rowblack} \multicolumn{1}{l|}{Original (zero-shot)} & 52.63 & 80.77 & \multicolumn{1}{l|}{87.41} & 56.76 & 83.99 & \multicolumn{1}{l|}{90.7} & 59.53 & 87.47 & \multicolumn{1}{l|}{93.79} & 56.23 & 81.83 & 89.26 \\
        \\
%

        %
         & \multicolumn{3}{c}{Paper {\scriptsize (9,521)}} & \multicolumn{3}{c}{Pavement {\scriptsize (18,311)}} & \multicolumn{3}{c}{Road {\scriptsize (15,402)}} & \multicolumn{3}{c}{Sea {\scriptsize (6,598)}} \\
        \multicolumn{1}{l|}{} & R@1 & R@5 & \multicolumn{1}{l|}{R@10} & R@1 & R@5 & \multicolumn{1}{l|}{R@10} & R@1 & R@5 & \multicolumn{1}{l|}{R@10} & R@1 & R@5 & R@10 \\ \midrule
        
         \multicolumn{1}{l|}{Full Fine-tune} & 69.96 & {\ul 92.94} & \multicolumn{1}{l|}{{\bf 98.39}} & 62.38 & 86.43 & \multicolumn{1}{l|}{{\ul 92.26}} & 60.73 & 84.17 & \multicolumn{1}{l|}{90.56} & 53.42 & {\ul 79.11} & 84.25 \\
        
         \multicolumn{1}{l|}{Last Layers Fine-tune} & 70.16 & {\bf 93.15} & \multicolumn{1}{l|}{{\ul 97.38}} & {\bf 64.29} & 85.71 & \multicolumn{1}{l|}{{\bf 92.74}} & {\bf 62.25} & {\ul 85.08} & \multicolumn{1}{l|}{{\ul 91.02}} & {\bf 57.53} & {\ul 79.11} & {\bf 85.62} \\
        
         \multicolumn{1}{l|}{LoRA} & {\bf 71.57} & {\ul 92.94} & \multicolumn{1}{l|}{96.98} & {\ul 63.33} & {\bf 87.14} & \multicolumn{1}{l|}{{\bf 92.74}} & 60.73 & {\bf 85.54} & \multicolumn{1}{l|}{{\bf 91.32}} & 54.45 & {\bf 80.14} & {\ul 84.59} \\
        
        \rowcolor{\rowlightgray} \multicolumn{1}{l|}{\ourspT} & {\ul 70.97} & 92.54 & \multicolumn{1}{l|}{97.18} & 62.74 & {\ul 86.9} & \multicolumn{1}{l|}{{\ul 92.26}} & {\ul 61.19} & 84.78 & \multicolumn{1}{l|}{{\ul 91.02}} & {\ul 56.51} & {\bf 80.14} & 83.9 \\
        
        \rowcolor{\rowdarkgray} \multicolumn{1}{l|}{\oursT} & 70.56 & 91.73 & \multicolumn{1}{l|}{96.57} & 61.55 & {\ul 86.9} & \multicolumn{1}{l|}{92.14} & 61.04 & 83.56 & \multicolumn{1}{l|}{90.56} & 55.82 & 78.42 & {\ul 84.59} \\
        
        \rowcolor{\rowblack} \multicolumn{1}{l|}{Linear Probing} & 69.76 & 91.33 & \multicolumn{1}{l|}{95.97} & 61.43 & 85.0 & \multicolumn{1}{l|}{91.55} & 59.51 & 82.65 & \multicolumn{1}{l|}{90.26} & 54.45 & 78.08 & 82.19 \\
        
        \rowcolor{\rowblack} \multicolumn{1}{l|}{Original (zero-shot)} & 67.74 & 89.92 & \multicolumn{1}{l|}{95.56} & 57.62 & 82.98 & \multicolumn{1}{l|}{89.4} & 54.49 & 80.37 & \multicolumn{1}{l|}{88.13} & 48.29 & 76.37 & 81.16 \\
        \\
%

        %
         & \multicolumn{3}{c}{Sky {\scriptsize (31,808)}} & \multicolumn{3}{c}{Table {\scriptsize (16,282)}} & \multicolumn{3}{c}{Tree {\scriptsize (36,466)}} & \multicolumn{3}{c}{Window {\scriptsize (14,209)}} \\
        \multicolumn{1}{l|}{} & R@1 & R@5 & \multicolumn{1}{l|}{R@10} & R@1 & R@5 & \multicolumn{1}{l|}{R@10} & R@1 & R@5 & \multicolumn{1}{l|}{R@10} & R@1 & R@5 & R@10 \\ \midrule
        
         \multicolumn{1}{l|}{Full Fine-tune} & 57.06 & 83.91 & \multicolumn{1}{l|}{91.46} & 65.3 & 89.18 & \multicolumn{1}{l|}{{\bf 94.99}} & 57.05 & 83.74 & \multicolumn{1}{l|}{90.23} & 70.91 & 92.87 & 96.53 \\
        
         \multicolumn{1}{l|}{Last Layers Fine-tune} & {\ul 59.42} & 84.82 & \multicolumn{1}{l|}{{\bf 91.69}} & {\bf 66.36} & {\bf 90.5} & \multicolumn{1}{l|}{{\bf 94.99}} & {\bf 59.02} & {\bf 85.11} & \multicolumn{1}{l|}{{\ul 91.15}} & 71.87 & {\ul 93.45} & {\ul 96.92} \\
        
         \multicolumn{1}{l|}{LoRA} & 59.27 & {\bf 85.58} & \multicolumn{1}{l|}{{\ul 91.53}} & 65.7 & 89.45 & \multicolumn{1}{l|}{{\ul 94.72}} & 57.7 & 84.2 & \multicolumn{1}{l|}{{\bf 91.21}} & {\bf 73.8} & {\bf 93.83} & {\ul 96.92} \\
        
        \rowcolor{\rowlightgray} \multicolumn{1}{l|}{\ourspT} & {\bf 59.73} & {\ul 85.13} & \multicolumn{1}{l|}{91.38} & {\ul 66.23} & {\ul 89.84} & \multicolumn{1}{l|}{94.33} & {\ul 57.9} & {\ul 84.79} & \multicolumn{1}{l|}{90.69} & {\ul 73.41} & 93.26 & {\bf 97.11} \\
        
        \rowcolor{\rowdarkgray} \multicolumn{1}{l|}{\oursT} & 58.73 & 84.06 & \multicolumn{1}{l|}{90.69} & 65.57 & 89.18 & \multicolumn{1}{l|}{{\bf 94.99}} & 56.33 & 83.74 & \multicolumn{1}{l|}{90.62} & 71.1 & 92.49 & {\bf 97.11} \\
        
        \rowcolor{\rowblack} \multicolumn{1}{l|}{Linear Probing} & 56.98 & 83.6 & \multicolumn{1}{l|}{90.39} & 62.4 & 87.6 & \multicolumn{1}{l|}{94.06} & 55.54 & 83.15 & \multicolumn{1}{l|}{90.1} & 68.79 & 92.49 & 96.53 \\
        
        \rowcolor{\rowblack} \multicolumn{1}{l|}{Original (zero-shot)} & 52.78 & 80.32 & \multicolumn{1}{l|}{87.72} & 59.37 & 83.25 & \multicolumn{1}{l|}{92.74} & 51.15 & 79.67 & \multicolumn{1}{l|}{88.26} & 67.44 & 91.33 & 95.57 \\
 \bottomrule
%
\end{tabular}
  }
\end{table*}


==> tables/subcoco_clip.tex <==
\begin{table*}[ht]
\centering
% \small
\caption{Performance comparison using the CLIP backbone on different COCO sub-domain splits. Each domain corpus was collected based on human-annotated objects within the images (number of training images in parentheses). Our adapters achieve performance on par with LoRA.
}
\label{tab:sub_coco_clip}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lllllllllllll@{}}
\toprule
 %
         & \multicolumn{3}{c}{Building {\scriptsize (23,021)}} & \multicolumn{3}{c}{Furniture {\scriptsize (17,882)}} & \multicolumn{3}{c}{Grass {\scriptsize (22,575)}} & \multicolumn{3}{c}{Metal {\scriptsize (22,526)}} \\
        \multicolumn{1}{l|}{} & R@1 & R@5 & \multicolumn{1}{l|}{R@10} & R@1 & R@5 & \multicolumn{1}{l|}{R@10} & R@1 & R@5 & \multicolumn{1}{l|}{R@10} & R@1 & R@5 & R@10 \\ \midrule
        
         \multicolumn{1}{l|}{Full Fine-tune} & 47.18 & 77.6 & \multicolumn{1}{l|}{87.22} & 48.9 & 78.81 & \multicolumn{1}{l|}{87.92} & 53.75 & 83.4 & \multicolumn{1}{l|}{91.54} & 49.35 & 76.46 & 85.89 \\
        
         \multicolumn{1}{l|}{Last Layers Fine-tune} & {\bf 54.11} & {\ul 80.08} & \multicolumn{1}{l|}{{\bf 89.89}} & 56.57 & {\bf 83.7} & \multicolumn{1}{l|}{{\ul 90.51}} & {\ul 58.78} & {\bf 87.26} & \multicolumn{1}{l|}{{\bf 94.0}} & {\bf 56.16} & {\bf 82.38} & {\bf 90.23} \\
        
         \multicolumn{1}{l|}{LoRA} & {\ul 53.32} & {\bf 80.77} & \multicolumn{1}{l|}{{\ul 88.4}} & {\bf 58.2} & {\ul 83.51} & \multicolumn{1}{l|}{{\bf 91.28}} & {\bf 59.21} & {\ul 86.08} & \multicolumn{1}{l|}{{\bf 94.0}} & {\ul 55.61} & {\ul 80.87} & {\ul 89.06} \\
        
        \rowcolor{\rowlightgray} \multicolumn{1}{l|}{\ourspT} & 52.43 & 78.79 & \multicolumn{1}{l|}{87.41} & {\ul 56.95} & 82.36 & \multicolumn{1}{l|}{90.12} & 55.46 & 84.9 & \multicolumn{1}{l|}{{\ul 92.72}} & 54.3 & 79.49 & 87.68 \\
        
        \rowcolor{\rowdarkgray} \multicolumn{1}{l|}{\oursT} & 49.75 & 75.62 & \multicolumn{1}{l|}{83.85} & 52.73 & 79.29 & \multicolumn{1}{l|}{88.69} & 52.03 & 81.26 & \multicolumn{1}{l|}{89.72} & 49.55 & 76.19 & 84.31 \\
        
        \rowcolor{\rowblack} \multicolumn{1}{l|}{Linear Probing} & 46.78 & 73.24 & \multicolumn{1}{l|}{83.55} & 52.83 & 78.91 & \multicolumn{1}{l|}{87.34} & 52.03 & 80.19 & \multicolumn{1}{l|}{89.83} & 48.86 & 75.43 & 84.72 \\
        
        \rowcolor{\rowblack} \multicolumn{1}{l|}{Original (zero-shot)} & 35.88 & 61.15 & \multicolumn{1}{l|}{71.75} & 44.68 & 70.66 & \multicolumn{1}{l|}{79.77} & 40.36 & 67.67 & \multicolumn{1}{l|}{80.62} & 40.67 & 65.79 & 75.64 \\
        \\
%

        %
         & \multicolumn{3}{c}{Paper {\scriptsize (9,521)}} & \multicolumn{3}{c}{Pavement {\scriptsize (18,311)}} & \multicolumn{3}{c}{Road {\scriptsize (15,402)}} & \multicolumn{3}{c}{Sea {\scriptsize (6,598)}} \\
        \multicolumn{1}{l|}{} & R@1 & R@5 & \multicolumn{1}{l|}{R@10} & R@1 & R@5 & \multicolumn{1}{l|}{R@10} & R@1 & R@5 & \multicolumn{1}{l|}{R@10} & R@1 & R@5 & R@10 \\ \midrule
        
         \multicolumn{1}{l|}{Full Fine-tune} & 59.68 & 85.69 & \multicolumn{1}{l|}{93.35} & 54.76 & 81.43 & \multicolumn{1}{l|}{87.86} & 48.86 & 80.21 & \multicolumn{1}{l|}{87.37} & 43.15 & 69.86 & 80.82 \\
        
         \multicolumn{1}{l|}{Last Layers Fine-tune} & {\bf 65.12} & {\bf 89.11} & \multicolumn{1}{l|}{{\bf 95.77}} & 57.98 & {\ul 83.1} & \multicolumn{1}{l|}{88.93} & {\ul 56.77} & 79.91 & \multicolumn{1}{l|}{{\bf 89.19}} & {\ul 48.97} & {\bf 75.34} & {\bf 82.19} \\
        
         \multicolumn{1}{l|}{LoRA} & {\ul 63.51} & {\ul 88.1} & \multicolumn{1}{l|}{{\ul 94.76}} & {\bf 61.55} & {\bf 84.52} & \multicolumn{1}{l|}{{\bf 90.24}} & {\bf 58.75} & {\bf 81.58} & \multicolumn{1}{l|}{{\bf 89.19}} & {\bf 49.66} & {\ul 75.0} & {\ul 81.51} \\
        
        \rowcolor{\rowlightgray} \multicolumn{1}{l|}{\ourspT} & 61.29 & 87.7 & \multicolumn{1}{l|}{94.35} & {\ul 59.52} & 82.5 & \multicolumn{1}{l|}{{\ul 89.05}} & 55.86 & {\ul 80.82} & \multicolumn{1}{l|}{{\ul 88.13}} & 47.95 & 74.32 & 80.82 \\
        
        \rowcolor{\rowdarkgray} \multicolumn{1}{l|}{\oursT} & 59.07 & 86.29 & \multicolumn{1}{l|}{92.94} & 53.33 & 79.4 & \multicolumn{1}{l|}{85.71} & 53.58 & 77.17 & \multicolumn{1}{l|}{85.39} & 40.75 & 70.55 & 80.82 \\
        
        \rowcolor{\rowblack} \multicolumn{1}{l|}{Linear Probing} & 58.87 & 85.48 & \multicolumn{1}{l|}{91.94} & 52.38 & 78.93 & \multicolumn{1}{l|}{86.07} & 50.84 & 77.02 & \multicolumn{1}{l|}{83.71} & 42.81 & 70.89 & 78.42 \\
        
        \rowcolor{\rowblack} \multicolumn{1}{l|}{Original (zero-shot)} & 52.62 & 77.42 & \multicolumn{1}{l|}{86.69} & 40.95 & 65.95 & \multicolumn{1}{l|}{76.31} & 38.51 & 62.71 & \multicolumn{1}{l|}{73.36} & 36.3 & 59.93 & 71.23 \\
        \\
%

        %
         & \multicolumn{3}{c}{Sky {\scriptsize (31,808)}} & \multicolumn{3}{c}{Table {\scriptsize (16,282)}} & \multicolumn{3}{c}{Tree {\scriptsize (36,466)}} & \multicolumn{3}{c}{Window {\scriptsize (14,209)}} \\
        \multicolumn{1}{l|}{} & R@1 & R@5 & \multicolumn{1}{l|}{R@10} & R@1 & R@5 & \multicolumn{1}{l|}{R@10} & R@1 & R@5 & \multicolumn{1}{l|}{R@10} & R@1 & R@5 & R@10 \\ \midrule
        
         \multicolumn{1}{l|}{Full Fine-tune} & 47.44 & 77.12 & \multicolumn{1}{l|}{87.87} & 55.15 & 81.53 & \multicolumn{1}{l|}{88.65} & 46.43 & 77.9 & \multicolumn{1}{l|}{86.36} & 56.07 & 85.16 & 91.33 \\
        
         \multicolumn{1}{l|}{Last Layers Fine-tune} & {\bf 52.1} & {\bf 81.92} & \multicolumn{1}{l|}{{\bf 90.31}} & {\ul 58.71} & {\bf 85.62} & \multicolumn{1}{l|}{{\ul 91.82}} & {\ul 53.05} & {\bf 81.9} & \multicolumn{1}{l|}{{\bf 89.38}} & {\bf 65.9} & {\ul 88.44} & 94.61 \\
        
         \multicolumn{1}{l|}{LoRA} & {\ul 51.33} & {\ul 80.32} & \multicolumn{1}{l|}{{\ul 89.24}} & {\bf 59.63} & 83.25 & \multicolumn{1}{l|}{{\bf 92.35}} & {\bf 53.11} & {\ul 80.52} & \multicolumn{1}{l|}{{\ul 88.79}} & {\ul 64.93} & {\bf 88.63} & {\bf 95.38} \\
        
        \rowcolor{\rowlightgray} \multicolumn{1}{l|}{\ourspT} & 49.43 & 78.49 & \multicolumn{1}{l|}{87.87} & 57.39 & {\ul 83.77} & \multicolumn{1}{l|}{91.42} & 50.49 & 79.87 & \multicolumn{1}{l|}{87.08} & 64.35 & 88.05 & {\ul 95.18} \\
        
        \rowcolor{\rowdarkgray} \multicolumn{1}{l|}{\oursT} & 45.16 & 75.9 & \multicolumn{1}{l|}{85.43} & 54.22 & 81.13 & \multicolumn{1}{l|}{88.52} & 47.15 & 75.8 & \multicolumn{1}{l|}{84.66} & 59.92 & 86.51 & 93.06 \\
        
        \rowcolor{\rowblack} \multicolumn{1}{l|}{Linear Probing} & 43.17 & 73.91 & \multicolumn{1}{l|}{84.82} & 53.56 & 80.87 & \multicolumn{1}{l|}{88.65} & 45.31 & 74.56 & \multicolumn{1}{l|}{83.34} & 59.92 & 86.13 & 93.06 \\
        
        \rowcolor{\rowblack} \multicolumn{1}{l|}{Original (zero-shot)} & 34.86 & 61.4 & \multicolumn{1}{l|}{73.07} & 44.46 & 72.3 & \multicolumn{1}{l|}{80.47} & 35.74 & 61.64 & \multicolumn{1}{l|}{73.31} & 50.87 & 80.15 & 87.86 \\

 \bottomrule
%
\end{tabular}
  }
\end{table*}

